Open book decompositions of fibre sums in contact topology

In the present paper we describe compatible open books for the fibre connected sum along binding components of open books, as well as for the fibre connected sum along multi-sections of open books. As an application the first description provides simple ways of constructing open books supporting all tight contact structures on $T^3$, recovering a result by van Horn-Morris, as well as an open book supporting the result of a Lutz twist along a binding component of an open book, recovering a result by Ozbagci--Pamuk.

==> bib.ltb.tex <==
\bib{Ale-SystemsOfKnottedCurves}{article}{
   author={Alexander, J.~W.},
   title={A lemma on systems of knotted curves},
 %  language={English, with French summary},
   journal={Proc. Nat. Acad. Sci. U.S.A.},
   volume={9},
   date={1923}
%   number={1-2},
   pages={93--95}
%   issn={0373-0956},
%   review={\MR{1162559 (93k:57029)}},
}

\bib{2012arXiv1204.3145}{article}{
	author = {Avdek, R.}
  title = {Liouville hypersurfaces and connect sum cobordisms},
 journal = {ArXiv e-prints},
%	archivePrefix = {arXiv},
   eprint = {arXiv:1204.3145}
% keywords = {Mathematics - Symplectic Geometry, Mathematics - Geometric Topology, 57R17, 53D10},
     year = {2012}
%    month = {may},
%   adsurl = {http://adsabs.harvard.edu/abs/2010arXiv1005.1978B},
%  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

\bib{2010arXiv1005.1978B}{article}{
	author = {Baker, K.~L.}
	author = {Etnyre, J.~B.}
	author = {Van Horn-Morris, J.},
    title = {Cabling, contact structures and mapping class monoids},
 journal = {ArXiv e-prints},
%	archivePrefix = {arXiv},
   eprint = {arXiv:1005.1978}
% keywords = {Mathematics - Symplectic Geometry, Mathematics - Geometric Topology, 57R17, 53D10},
     year = {2010}
%    month = {may},
%   adsurl = {http://adsabs.harvard.edu/abs/2010arXiv1005.1978B},
%  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

\bib{arXiv1005.2169v1}{article}{
   author={Baldwin, J.~A.},
   title={Contact monoids and Stein cobordisms},
 journal = {ArXiv e-prints},
   eprint = {arXiv:1005.2169v1}
   date={2010}
}

\bib{MR2385640}{article}{
   author={Baldwin, J.~A.},
   title={Comultiplicativity of the Ozsv\'ath-Szab\'o contact invariant},
   journal={Math. Res. Lett.},
   volume={15},
   date={2008},
%   number={2},
   pages={273--287}
%   issn={1073-2780}
%   review={\MR{2385640 (2009c:57043)}},
}

\bib{MR1447038}{article}{
   author={Colin, Vincent},
   title={Chirurgies d'indice un et isotopies de sph\`eres dans les
   vari\'et\'es de contact tendues},
 %  language={French, with English and French summaries},
   journal={C. R. Acad. Sci. Paris S\'er. I Math.},
   volume={324},
   date={1997},
%   number={6},
   pages={659--663}
%   issn={0764-4442},
%   review={\MR{1447038 (98e:57036)}},
%   doi={10.1016/S0764-4442(97)86985-6},
}

\bib{El20years}{article}{
   author={Eliashberg, Y.},
   title={Contact $3$-manifolds twenty years since J. Martinet's work},
 %  language={English, with French summary},
   journal={Ann. Inst. Fourier (Grenoble)},
   volume={42},
   date={1992}
%   number={1-2},
   pages={165--192}
%   issn={0373-0956},
%   review={\MR{1162559 (93k:57029)}},
}

\bib{MR1162559}{article}{
   author={Eliashberg, Y.},
   title={Contact $3$-manifolds twenty years since J. Martinet's work},
   language={English, with French summary},
   journal={Ann. Inst. Fourier (Grenoble)},
   volume={42},
   date={1992},
%   number={1-2},
   pages={165--192}
%   issn={0373-0956},
%   review={\MR{1162559 (93k:57029)}},
}


\bib{MR1022310}{article}{
   author={Eliashberg, Y.},
   title={Classification of overtwisted contact structures on $3$-manifolds},
   journal={Invent. Math.},
   volume={98},
   date={1989},
%   number={3},
   pages={623--637}
%   issn={0020-9910},
%   review={\MR{1022310 (90k:53064)}},
%   doi={10.1007/BF01393840},
}

\bib{MR2023279}{article}{
   author={Eliashberg, Y.},
   title={A few remarks about symplectic filling},
   journal={Geom. Topol.},
   volume={8},
   date={2004},
   pages={277--293}
%   issn={1465-3060},
%   review={\MR{2023279 (2005a:57022b)}},
%   doi={10.2140/gt.2004.8.277},
}

\bib{MR2496415}{article}{
   author={Eliashberg, Yakov},
   author={Fraser, Maia},
   title={Topologically trivial Legendrian knots},
   journal={J. Symplectic Geom.},
   volume={7},
   date={2009},
%   number={2},
   pages={77--127},
   issn={1527-5256},
   review={\MR{2496415 (2010d:57024)}},
}


\bib{EliFraTTLK}{article}{
   author={Eliashberg, Y.},
   author={Fraser, M.},
   title={Topologically trivial Legendrian knots},
   journal={J. Symplectic Geom.},
   volume={7},
   date={2009},
%   number={2},
   pages={77--127}
%   issn={1527-5256},
%   review={\MR{2496415 (2010d:57024)}},
}

\bib{MR1044658}{article}{
   author={Eliashberg, Y.},
   title={Topological characterization of Stein manifolds of dimension
   $>2$},
   journal={Internat. J. Math.},
   volume={1},
   date={1990},
%   number={1},
   pages={29--46}
%   issn={0129-167X},
%   review={\MR{1044658 (91k:32012)}},
%   doi={10.1142/S0129167X90000034},
}

\bib{MR1128541}{article}{
   author={Eliashberg, Yakov},
   author={Gromov, Mikhael},
   title={Convex symplectic manifolds},
   conference={
      title={Several complex variables and complex geometry, Part 2 (Santa
      Cruz, CA, 1989)},
   },
   book={
      series={Proc. Sympos. Pure Math.},
      volume={52},
      publisher={Amer. Math. Soc.},
      place={Providence, RI},
   },
   date={1991},
   pages={135--162},
   review={\MR{1128541 (93f:58073)}},
}


\bib{eliGro-convex_symplectic_manifolds}{article}{
   author={Eliashberg, Y.},
   author={Gromov, M.},
   title={Convex symplectic manifolds},
   conference={
      title={Several complex variables and complex geometry, Part 2 (Santa
      Cruz, CA, 1989)},
   },
   book={
      series={Proc. Sympos. Pure Math.},
      volume={52},
      publisher={Amer. Math. Soc.},
      place={Providence, RI},
   },
   date={1991},
   pages={135--162}
%   review={\MR{1128541 (93f:58073)}},
}

\bib{MR2249250}{article}{
   author = {Etnyre, J.~B.},
   title={Lectures on open book decompositions and contact structures},
   conference={
      title={Floer homology, gauge theory, and low-dimensional topology},
   },
   book={
      series={Clay Math. Proc.},
      volume={5},
      publisher={Amer. Math. Soc.},
      place={Providence, RI},
   },
   date={2006},
   pages={103--141}
%   review={\MR{2249250 (2007g:57042)}},
}

\bib{MR2407103}{article}{
   author = {Etnyre, J.~B.},
   title={On contact surgery},
   journal={Proc. Amer. Math. Soc.},
   volume={136},
   date={2008},
%   number={9},
   pages={3355--3362}
%   issn={0002-9939},
%   review={\MR{2407103 (2010b:57036)}},
%   doi={10.1090/S0002-9939-08-09278-2},
}

\bib{2010arXiv1012.3745E}{article}{
   author = {Etnyre, J.~B.},
    title = {On knots in overtwisted contact structures},
  journal = {ArXiv e-prints},
  eprint={arXiv:1012.3745},
  date={2010}
}

\bib{etn-on_symplectic_cobordisms}{article}{
   author = {Etnyre, J.~B.},
      author = {Honda, K.},
    title = {On symplectic cobordisms}
}

\bib{MR2023278}{article}{
   author={Etnyre, John B.},
   title={On symplectic fillings},
   journal={Algebr. Geom. Topol.},
%   volume={4},
   date={2004},
   pages={73--80}
%   issn={1472-2747},
%   review={\MR{2023278 (2005a:57022a)}},
%   doi={10.2140/agt.2004.4.73},
}



\bib{etn-convex_notes}{article}{
   author = {Etnyre, J.~B.},
   title={Convex surfaces in contact geometry: Class notes},
   date={2004},
   eprint={http://people.math.gatech.edu/~etnyre/preprints/papers/surfaces.pdf}
}

\bib{MR2024641}{article}{
   author = {Etnyre, J.~B.},
   author={Ng, L.},
   title={Problems in low dimensional contact topology},
   conference={
      title={Topology and geometry of manifolds},
      address={Athens, GA},
      date={2001},
   },
   book={
      series={Proc. Sympos. Pure Math.},
      volume={71},
      publisher={Amer. Math. Soc.},
      place={Providence, RI},
   },
   date={2003},
   pages={337--357}
%   review={\MR{2024641 (2004k:57033)}},
}

\bib{2009arXiv0909.3465E}{article}{
   author = {Etnyre, J.~B.},
   author = {Shea Vela-Vick, D.},
    title = {Torsion and open book decompositions},
  journal = {ArXiv e-prints},
%archivePrefix = {arXiv},
   eprint = {arXiv:0909.3465},
% keywords = {Mathematics - Symplectic Geometry, Mathematics - Geometric Topology, 57M27, 57R58},
     year = {2009}
%    month = {sep},
%   adsurl = {http://adsabs.harvard.edu/abs/2009arXiv0909.3465E},
%  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

\bib{2009arXiv0909.3465E}{article}{
   author = {Etnyre, J.~B.},
   author = {Baker, K.~L.},
 		author={{Van Horn-Morris}, J.},
    title = {Cabling, contact structures and mapping class monoids},
         year = {2009},
       eprint = {arXiv:arXiv:0909.3465v1}
 journal = {ArXiv e-prints}
}


\bib{FucTab1}{article}{
   author = {Fuchs, D.},
   author = {Tabachnikov, S.},
    title = {Invariants of Legendrian and transverse knots in the standard 
contact space}
}

\bib{MR2350472}{article}{
   author = {Gay, D.~T.},
   author = {Kirby, R.},
   title={Constructing Lefschetz-type fibrations on four-manifolds},
   journal={Geom. Topol.},
   volume={11},
   date={2007},
   pages={2075--2115}
%   issn={1465-3060}
}

\bib{2009arXiv0908.3774G}{article}{
   author = {Gay, D.~T.},
   author = {Stipsicz, A.~I.},
    title = {On symplectic caps},
  journal = {ArXiv e-prints},
   eprint = {arxiv:0908.3774},
% keywords = {Mathematics - Symplectic Geometry, Mathematics - Geometric Topology},
     year = {2009}
%   adsurl = {http://adsabs.harvard.edu/abs/2009arXiv0908.3774G},
%  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




\bib{MR2397738}{book}{
   author={Geiges, H.},
   title={An Introduction to Contact Topology},
   series={Cambridge Studies in Advanced Mathematics},
   volume={109},
   publisher={Cambridge University Press},
   place={Cambridge},
   date={2008},
   pages={xvi+440}
%   isbn={978-0-521-86585-2},
%   review={\MR{2397738 (2008m:57064)}},
%   doi={10.1017/CBO9780511611438},
}

\bib{2003math......3303G}{article}{
   author={Geiges, H.},
   author={Gonzalo, J.},
   title={On the topology of the space of contact structures on torus
   bundles},
   journal={Bull. London Math. Soc.},
   volume={36},
   date={2004},
%   number={5},
   pages={640--646}
%   issn={0024-6093},
%   review={\MR{2070440 (2005f:53153)}},
%   doi={10.1112/S0024609304003376},
}

\bib{MR2070440}{article}{
   author={Geiges, H.},
   author={Gonzalo, J.},
   title={On the topology of the space of contact structures on torus
   bundles},
   journal={Bull. London Math. Soc.},
   volume={36},
   date={2004},
%   number={5},
   pages={640--646}
%   issn={0024-6093},
%   review={\MR{2070440 (2005f:53153)}},
%   doi={10.1112/S0024609304003376},
}

\bib{GeiGon-15YearsOfContactSpheres}{article}{
   author={Geiges, H.},
    author= {Gonzalo, J.},
    title = {Fifteen years of contact circles and contact spheres},
  journal = {unpublished}
}

\bib{2009arXiv0903.1488D}{article}{
   author={Ding, F.},
   author={Geiges, H.},
    title = {The diffeotopy group of S\^{}1 $\backslash$times S\^{}2 via contact topology},
  journal = {ArXiv e-prints},
	date = {2009}
}

\bib{MR2455948}{article}{
   author={Ding, F.},
   author={Geiges, H.},
   title={A unique decomposition theorem for tight contact 3-manifolds},
   journal={Enseign. Math. (2)},
   volume={53},
   date={2007},
%   number={3-4},
   pages={333--345}
%   issn={0013-8584},
%   review={\MR{2455948 (2009k:57042)}},
}


\bib{2010arXiv1012.1721G}{article}{
   author={Ding, F.},
   author={Geiges, H.},
    title = {Neighbourhoods and isotopies of knots in contact $3$-manifolds},
%  eprint= {arXiv:1012.1721},
%  	date = {2010},
  	  journal={Arch. Math. (Basel)},
   volume={97},
   date={2011},
   pages={391--397}
}

\bib{MR1823497}{article}{
   author={Ding, F.},
   author={Geiges, H.},
   title={Symplectic fillability of tight contact structures on torus
   bundles},
   journal={Algebr. Geom. Topol.},
   volume={1},
   date={2001},
   pages={153--172 }
%   issn={1472-2747},
%   review={\MR{1823497 (2002b:53134)}},
%   doi={10.2140/agt.2001.1.153},
}


\bib{MR2056760}{article}{
   author={Ding, F.},
   author={Geiges, H.},
   author={Stipsicz, A.~I.},
   title={Surgery diagrams for contact $3$-manifolds},
   journal={Turkish J. Math.},
   volume={28},
   date={2004},
%   number={1},
   pages={41--74}
%   issn={1300-0098},
%   review={\MR{2056760 (2005c:57028)}},
}


\bib{MR2225643}{article}{
   author={Ghiggini, P.},
   title={Linear Legendrian curves in $T^3$},
   journal={Math. Proc. Cambridge Philos. Soc.},
   volume={140},
   date={2006},
%   number={3},
   pages={451--473}
%   issn={0305-0041},
%   review={\MR{2225643 (2007a:57031)}},
%   doi={10.1017/S0305004105009151},
}



\bib{MR2180909}{article}{
   author={Ghiggini, P.},
   author={Lisca, P.},
   author={Stipsicz, Andr{\'a}s I.},
   title={Classification of tight contact structures on small Seifert
   3-manifolds with $e_0\geq 0$},
   journal={Proc. Amer. Math. Soc.},
   volume={134},
   date={2006},
%   number={3},
   pages={909--916 }
%   issn={0002-9939},
%   review={\MR{2180909 (2006m:57036)}},
%   doi={10.1090/S0002-9939-05-08013-5},
}
	

\bib{MR1957051}{article}{
   author={Giroux, E.},
   title={G\'eom\'etrie de contact: de la dimension trois vers les
   dimensions sup\'erieures},
%   language={French, with French summary},
   conference={
      title={},
      address={Beijing},
      date={2002},
   },
   book={
      publisher={Higher Ed. Press},
      place={Beijing},
   },
   date={2002},
   pages={405--414}
%   review={\MR{1957051 (2004c:53144)}},
}

\bib{MR2511589}{article}{
   author={Colin, V.},
   author={Giroux, E.},
   author={Honda, K.},
   title={Finitude homotopique et isotopique des structures de contact
   tendues},
%   language={French, with French summary},
   journal={Publ. Math. Inst. Hautes \'Etudes Sci.},
%   number={109},
   date={2009},
   pages={245--293}
%   issn={0073-8301},
%   review={\MR{2511589 (2010g:53167)}},
%   doi={10.1007/s10240-009-0022-y},
}



\bib{2001math......2009G}{article}{
   author={Giroux, E.},
    title = {Sur les transformations de contact au-dessus des surfaces},
%  journal = {ArXiv Mathematics e-prints},
   eprint = {arXiv:math/0102009},
% keywords = {Geometric Topology, Symplectic Geometry, Differential Geometry, 57M50, 57R17 (primary) 53D35, 53D10 (secondary)},
     year = {2001}
%   adsurl = {http://adsabs.harvard.edu/abs/2001math......2009G},
%  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

\bib{1999math.....11235G}{article}{
   author={Giroux, E.},
    title = {Structures de contact sur les varietes fibrees en cercles au-dessus d'une surface},
%  journal = {ArXiv Mathematics e-prints},
   eprint = {arXiv:math/9911235},
% keywords = {Mathematics - Geometric Topology, Mathematics - Differential Geometry, Mathematics - Symplectic Geometry, 57M50, 57R17 (primary) 53D35, 53D10 (secondary)},
     year = {1999}
%    month = nov,
%   adsurl = {http://adsabs.harvard.edu/abs/1999math.....11235G},
%  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

\bib{MR1129802}{article}{
   author={Giroux, E.},
   title={Convexit\'e en topologie de contact},
%   language={French},
   journal={Comment. Math. Helv.},
   volume={66},
   date={1991},
%   number={4},
   pages={637--677}
%   issn={0010-2571},
%   review={\MR{1129802 (93b:57029)}},
%   doi={10.1007/BF02566670},
}

\bib{MR1779622}{article}{
   author={Giroux, E.},
   title={Structures de contact en dimension trois et bifurcations des
   feuilletages de surfaces},
%   language={French},
   journal={Invent. Math.},
   volume={141},
   date={2000},
%   number={3},
   pages={615--689}
%   issn={0020-9910},
%   review={\MR{1779622 (2001i:53147)}},
%   doi={10.1007/s002220000082},
}



\bib{MR2207791}{article}{
   author={Giroux, E.},
   author={Goodman, N.},
   title={On the stable equivalence of open books in three-manifolds},
   journal={Geom. Topol.},
%   volume={10},
   date={2006},
   pages={97--114}
%   issn={1465-3060},
%   review={\MR{2207791 (2006k:57046)}},
%   doi={10.2140/gt.2006.10.97},
}
		




\bib{MR2171807}{article}{
   author={Goodman, N.},
   title={Overtwisted open books from sobering arcs},
   journal={Algebr. Geom. Topol.},
   volume={5},
   date={2005},
   pages={1173--1195}
%   issn={1472-2747},
%   review={\MR{2171807 (2006h:57022)}},
%   doi={10.2140/agt.2005.5.1173},
}



\bib{MR0098847}{article}{
   author={Grauert, H.},
   title={On Levi's problem and the imbedding of real-analytic manifolds},
   journal={Ann. of Math. (2)},
   volume={68},
   date={1958},
   pages={460--472}
%   issn={0003-486X},
%   review={\MR{0098847 (20 \#5299)}},
}
		



\bib{MR1940409}{article}{
   author={Honda, K.},
   title={Gluing tight contact structures},
   journal={Duke Math. J.},
   volume={115},
   date={2002},
%   number={3},
   pages={435--478}
%   issn={0012-7094},
%   review={\MR{1940409 (2003i:53125)}},
%   doi={10.1215/S0012-7094-02-11532-4},
}

\bib{MR1786111}{article}{
   author={Honda, K.},
   title={On the classification of tight contact structures. I},
   journal={Geom. Topol.},
   volume={4},
   date={2000},
   pages={309--368}
%   issn={1465-3060},
%   review={\MR{1786111 (2001i:53148)}},
%   doi={10.2140/gt.2000.4.309},
}

\bib{hon-tight-classification-1}{article}{
   author={Honda, K},
   title={On the classification of tight contact structures. I},
   journal={Geom. Topol.},
   volume={4},
   date={2000},
   pages={309--368}
%   issn={1465-3060},
%   review={\MR{1786111 (2001i:53148)}},
%   doi={10.2140/gt.2000.4.309},
}

\bib{2008arXiv0807.2431H}{article}{
   author = {Honda, K.},
   author = {Kazez, W.~H.},
   author = {Matic, G.},
    title = {Contact structures, sutured Floer homology and TQFT},
  eprint = {arXiv:0807.2431},
     date = {2008}
}
\bib{2007arXiv0705.2828H}{article}{
   author = {Honda, K.},
   author = {Kazez, W.~H.},
   author = {Matic, G.},
    title = {The contact invariant in sutured Floer homology},
  eprint = {	arXiv:0705.2828},
     date = {2007}
}

\bib{MR1874319}{article}{
   author={Honda, Ko},
   author={Kazez, William H.},
   author={Mati{\'c}, Gordana},
   title={Convex decomposition theory},
   journal={Int. Math. Res. Not.},
   date={2002},
%   number={2},
   pages={55--88}
%   issn={1073-7928},
%   review={\MR{1874319 (2002k:57064)}},
%   doi={10.1155/S1073792802101140},
}


\bib{2009arXiv0910.4382J}{article}{
   author = {Juh\'{a}sz, A.},
    title = {Cobordisms of sutured manifolds},
  journal = {ArXiv e-prints},
   eprint = {arXiv:0910.4382},
  	year  = {2009}
%   adsurl = {http://adsabs.harvard.edu/abs/2009arXiv0910.4382J},
%  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

\bib{MR2253454}{article}{
   author={Juh{\'a}sz, A.},
   title={Holomorphic discs and sutured manifolds},
   journal={Algebr. Geom. Topol.},
   volume={6},
   date={2006},
   pages={1429--1457}
%   issn={1472-2747},
%   review={\MR{2253454 (2007g:57024)}},
%   doi={10.2140/agt.2006.6.1429},
}





\bib{MR1487723}{article}{
   author={Kanda, Y.},
   title={The classification of tight contact structures on the $3$-torus},
   journal={Comm. Anal. Geom.},
   volume={5},
   date={1997},
%   number={3},
   pages={413--438}
%   issn={1019-8385},
%   review={\MR{1487723 (99c:57054)}},
}

\bib{MR1632790}{article}{
   author={Kanda, Y.},
   title={On the Thurston-Bennequin invariant of Legendrian knots and
   nonexactness of Bennequin's inequality},
   journal={Invent. Math.},
   volume={133},
   date={1998},
%   number={2},
   pages={227--242}
%   issn={0020-9910},
%   review={\MR{1632790 (99g:57030)}},
%   doi={10.1007/s002220050245},
}



\bib{MR1487723}{article}{
   author={Kanda, Y.},
   title={The classification of tight contact structures on the $3$-torus},
   journal={Comm. Anal. Geom.},
   volume={5},
   date={1997},
%   number={3},
   pages={413--438}
%   issn={1019-8385},
%   review={\MR{1487723 (99c:57054)}},
}

\bib{Klukas-Thesis}{article}{
   author={Klukas, M.},
   title={Constructions of open book decompositions and applications of convex surfaces in contact topology},
   journal={Dissertation, University of Cologne, Germany},
   %eprint = {http://www.aimath.org/~jvanhorn/dissertation-jvhm.pdf},
   date={submitted March 2012}
}

		
\bib{MassotThesis}{article}{
   author={Massot, P.},
   title={Thesis - Sur\ldots}
}

\bib{2009arXiv0912.5107M}{article}{
   author = {Massot, P.},
    title = {Infinitely many universally tight torsion free contact structures with vanishing Ozsv\'ath-Szab\'o contact invariants},
  journal = {ArXiv e-prints},
%archivePrefix = {arXiv},
eprint = {arXiv:0912.5107},
     year = {2009}
%    month = {dec},
%   adsurl = {http://adsabs.harvard.edu/abs/2009arXiv0912.5107M},
%  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

\bib{MR1487640}{book}{
   author={Milnor, J.~W.},
   title={Topology from the Differentiable Viewpoint},
   series={Princeton Landmarks in Mathematics},
%   note={Based on notes by David W. Weaver;
%   Revised reprint of the 1965 original},
   publisher={Princeton University Press},
   place={Princeton, NJ},
   date={1997},
   pages={xii+64}
%   isbn={0-691-04833-9},
%   review={\MR{1487640 (98h:57051)}},
}



\bib{2009arXiv0905.0986O}{article}{
   author = {Ozbagci, B.},
   author = {Pamuk, M.},
    title = {Full Lutz twist along the binding of an open book},
  journal = {ArXiv e-prints},
%archivePrefix = {arXiv},
   eprint = {arXiv:0905.0986},
% keywords = {Mathematics - Geometric Topology, 57R17},
     year = {2009}
%    month = {may},
%   adsurl = {http://adsabs.harvard.edu/abs/2009arXiv0905.0986O},
%  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

\bib{MR1414898}{book}{
   author={Prasolov, V.~V.},
   author={Sossinsky, A.~B.},
   title={Knots, Links, Braids and $3$-Manifolds},
   series={Translations of Mathematical Monographs},
   volume={154},
%   note={An introduction to the new invariants in low-dimensional topology;
%   Translated from the Russian manuscript by Sossinsky [Sosinski\u\i]},
   publisher={American Mathematical Society},
   place={Providence, RI},
   date={1997},
   pages={viii+239}
%   isbn={0-8218-0588-6},
%   review={\MR{1414898 (98i:57018)}},
}



\bib{vanHornMorris-Thesis}{article}{
   author={{Van Horn-Morris}, J.},
   title={Constructions of open book decompositions},
   journal={Dissertation, University of Texas at Austin},
   eprint = {http://www.aimath.org/~jvanhorn/dissertation-jvhm.pdf},
   date={2007}
}

\bib{MR0375366}{article}{
   author={Thurston, W.~P.},
   author={Winkelnkemper, H.~E.},
   title={On the existence of contact forms},
   journal={Proc. Amer. Math. Soc.},
   volume={52},
   date={1975},
   pages={345--347}
%   issn={0002-9939},
%   review={\MR{0375366 (51 \#11561)}},
}

\bib{MR1114405}{article}{
   author={Weinstein, A.},
   title={Contact surgery and symplectic handlebodies},
   journal={Hokkaido Math. J.},
   volume={20},
   date={1991},
%   number={2},
   pages={241--251}
%   issn={0385-4035},
%   review={\MR{1114405 (92g:53028)}},
}

\bib{2010arXiv1009.2746W}{article}{
   author = {Wendl, C.},
    title = {A hierarchy of local symplectic filling obstructions for contact $3$-manifolds},
  journal = {ArXiv e-prints},
%archivePrefix = {arXiv},
   eprint = {arXiv:1009.2746},
   date = {2010}
% yearsurl = {ttp://adsabs.harvard.edu/abs/2010arXiv1009.2746W}
}




\bib{2010arXiv1010.3496Z}{article}{
   author = {Zarev, R.},
    title = {Joining and gluing sutured Floer homology},
  journal = {ArXiv e-prints},
 keywords = {Mathematics - Geometric Topology, Mathematics - Symplectic Geometry, 57R58, 57M27},
     date = {2010}
}


